MACQ: A Holistic View of Model Acquisition Techniques

For over three decades, the planning community has explored countless methods for data-driven model acquisition. These range in sophistication (e.g., simple set operations to full-blown reformulations), methodology (e.g., logic-based vs. planing-based), and assumptions (e.g., fully vs. partially observable). With no fewer than 43 publications in the space, it can be overwhelming to understand what approach could or should be applied in a new setting. We present a holistic characterization of the action model acquisition space and further introduce a unifying framework for automated action model acquisition. We have re-implemented some of the landmark approaches in the area, and our characterization of all the techniques offers deep insight into the research opportunities that remain; i.e., those settings where no technique is capable of solving.

==> section/2-background.tex <==
\clearpage
\section{Background}
\label{sec:background}

\begin{itemize}
    \item Observations (Bonet \& Geffner) <-- probably not, since we aren't going deep into the theory on this
    \item Terms for ``generation'', ``tokenization'', and ``extraction''.
    \item Intro PDDL.
    \item State traces.
    \item (maybe) SAT theories and knowledge compilation
\end{itemize}
